Low-Rank Projections of GCNs Laplacian

In this work, we study the behavior of standard models for community detection under spectral manipulations. Through various ablation experiments, we evaluate the impact of bandpass filtering on the performance of a GCN: we empirically show that most of the necessary and used information for nodes classification is contained in the low-frequency domain, and thus contrary to images, high frequencies are less crucial to community detection. In particular, it is sometimes possible to obtain accuracies at a state-of-the-art level with simple classifiers that rely only on a few low frequencies.

==> mathdef.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Paper dependent stuff    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Tau}{\mathcal{T}}
\newcommand{\OurAlgorithm}{\texttt{Robust-EPC}}
\newcommand{\ux}{\underline{x}}
\newcommand{\ox}{\overline{x}}
\newcommand{\bom}{\bm{\omega}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Aesthetics               %
% over-underline, hat, bold%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eps}{\varepsilon}
\newcommand{\vareps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
%\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}

\newcommand*{\MyDef}{\mathrm{\tiny def}}
\newcommand*{\eqdefU}{\ensuremath{\mathop{\overset{\MyDef}{=}}}}% Unscaled version
% \newcommand*{\eqdef}{\mathop{\overset{\MyDef}{\resizebox{\widthof{\eqdefU}}{\heightof{=}}{=}}}}
\newcommand{\eqdef}{\stackrel{def}{=}}


\def\:#1{\protect \ifmmode {\mathbf{#1}} \else {\textbf{#1}} \fi}
\newcommand{\CommaBin}{\mathbin{\raisebox{0.5ex}{,}}}

\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wo}[1]{\overline{#1}}
\newcommand{\wb}[1]{\overline{#1}}

% bf and bm missing due to conflict!!
\newcommand{\bsym}[1]{\mathbf{#1}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

% calligraphic
\newcommand{\cf}{\mathcal{f}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math jargon              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\defeq}{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand{\maxund}[1]{\max\limits_{#1}}
\newcommand{\supund}[1]{\text{sup}\limits_{#1}}
\newcommand{\minund}[1]{\min\limits_{#1}}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\bigotime}{\mathcal{O}}
\newcommand{\dd}{\mathrm{d}}

\DeclareMathOperator*{\argmin}{arg\,min} 
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\cupdot}{\mathbin{\mathaccent\cdot\cup}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Matrix operators         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\transpose}{^\mathsf{\scriptscriptstyle T}}
\newcommand{\transp}{\mathsf{\scriptscriptstyle T}}
\DeclareMathOperator{\Tr}{Tr}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Statistic operators      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\probability}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\probdist}{Pr}
\DeclareMathOperator*{\expectedvalue}{\mathbb{E}}
\DeclareMathOperator*{\variance}{\text{Var}}
\newcommand{\expectedvalueover}[1]{\expectedvalue\limits_{#1}}
\newcommand{\condbar}{\;\middle|\;}
\newcommand{\gaussdistr}{\mathcal{N}}
\newcommand{\uniformdistr}{\mathcal{U}}
\newcommand{\bernoullidist}{\mathcal{B}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algebraic Sets           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\statespace}{\mathcal{X}}
\newcommand{\funcspace}{\mathcal{F}}
\newcommand{\dynaspace}{\mathcal{T}}


\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\providecommand*\corollaryautorefname{Corollary}
\newtheorem{lemma}{Lemma}
\providecommand*\lemmaautorefname{Lemma}
\newtheorem{proposition}{Proposition}
\providecommand*\propositionautorefname{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{property}{Property}
\newtheorem{assumption}{Assumption}
\providecommand*\assumptionautorefname{Assumption}
\newtheorem{conjecture}{Conjecture}
\providecommand*\algorithmautorefname{Algorithm}

% \newtheorem*{definition*}{Definition}
% \newtheorem*{theorem*}{Theorem}
% \newtheorem*{proposition*}{Proposition}
% \newtheorem*{remark*}{Remark}
% \newtheorem*{example*}{Example}



==> work_hypothesis.tex <==
Our initial data are graph features $x\in \mathbb{R}^{K\times P}$ where $K$ is the size of a graph with adjacency matrix $\mathcal{A}\in \mathbb{R}^{K^2}$ and $P$ is the number of node-features. We consider GCNs as introduced in \citep{kipf2016semi}, which corresponds to Graph Neural Networks that propagate features graph input $x_0\triangleq x$ through a cascade of layers, via the iteration:
\begin{equation}
x_{n+1}\triangleq\sigma\bigg(A_\eta x_nW_n\bigg)\,,
\end{equation}

where $A_\eta$ is a linear operator obtained from the adjacency matrix $\mathcal{A}$ parametrized by $\eta$ a smoothness hyperparameter, $\sigma$ a point-wise non-linearity and $W_n$ a parametrized affine operator. In the semi-supervised setting, a final layer $x_N$ is fed to a supervised loss $\ell$ and $\{W_0,...,W_{N-1}\}$ are trained in an end-to-end manner to adjust the label of each node. In this setting, we let $\mathcal{D}$ be the diagonal matrix of vertex degree, and we consider the normalized Laplacian with self-loop $\eta$:
\begin{equation}
A_\eta\triangleq \frac{1}{\eta + 1} \left( \eta \mI+ \mathcal{D}^{-1/2}\mathcal{A}\mathcal{D}^{-1/2}\right) \,.
\end{equation}

Here, $A_\eta$ is normalized such that $\Vert A_\eta\Vert=1$, in order to avoid any side effects linked to a rescaling of the loss function. We remark that other smoohting $A_\eta$ have been proposed, however, we tried several different possibilities that did not affect substentially our numerical performances, thus we decided to keep the simplest formulation to be handled mathematically. Note also that ignoring $\mathcal{D}$, $\eta \mI+\mathcal{A}$ is often interpreted as a low-pass filter, as for a given feature $x=(x_i)_i$, it explicitely performs a local averaging of a node $i$:
\[\,[(\eta \mI+\mathcal{A})x]_i=\eta x_i+\sum_{j\rightarrow i}\mathcal{A}_{i,j}x_j\,.\]

We are interested in analyzing the properties of spectral approximations of $A_\eta$. We consider the set of eigen-values $\Lambda=\{\lambda_k\}_k$ of $\mathcal{D}^{-1/2}\mathcal{A}\mathcal{D}^{-1/2}$,  such that $\lambda_{k}> \lambda_{k+1}$, without their multiplicity, such that $\pi_\lambda$ is the orthogonal projector on the eigenspace of $\lambda$. We remind that $\Lambda \subset ]-1,1]$ and that $\lambda_1=1$ can be interpreted as the lowest frequency of the Laplacian. Since the adjacency matrix is normalized, the eigenvectors of $\lambda_1$ are the constant vectors of 1 supported on a connected component. We then note that:
\begin{equation}
A_\eta=\sum_{\lambda_k} \frac{\eta+\lambda_k}{\eta+1}\pi_{\lambda_k}\,.
\end{equation}

In this case, the spectrum of $A_\eta$ lays in $]\frac{\eta-1}{\eta+1},1]$. In our work, we are interested in studying projection operators $\Pi$ on $A_\eta$, of the type:
\begin{equation}
 \Pi(A_\eta)=\sum_{\lambda_k} \Pi(\lambda_k) \frac{\eta+\lambda_k}{\eta+1} \pi_{\lambda_k}\,.
 \end{equation}
 
The next section studies empirically the property of such approximations in the context of GCNs and simpler architectures.
